HybridReg: Robust 3D Point Cloud Registration with Hybrid Motions

Scene-level point cloud registration is very challenging when considering dynamic foregrounds. Existing indoor datasets mostly assume rigid motions, so the trained models cannot robustly handle scenes with non-rigid motions. On the other hand, non-rigid datasets are mainly object-level, so the trained models cannot generalize well to complex scenes. This paper presents HybridReg, a new approach to 3D point cloud registration, learning uncertainty mask to account for hybrid motions: rigid for backgrounds and non-rigid/rigid for instance-level foregrounds. First, we build a scene-level 3D registration dataset, namely HybridMatch, designed specifically with strategies to arrange diverse deforming foregrounds in a controllable manner. Second, we account for different motion types and formulate a mask-learning module to alleviate the interference of deforming outliers. Third, we exploit a simple yet effective negative log-likelihood loss to adopt uncertainty to guide the feature extraction and correlation computation. To our best knowledge, HybridReg is the first work that exploits hybrid motions for robust point cloud registration. Extensive experiments show HybridReg's strengths, leading it to achieve state-of-the-art performance on both widely-used indoor and outdoor datasets.

==> figures/tex/pipeline.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.995\linewidth]{figures/pdf/pipeline.pdf}
    \caption{Our framework: (i) \ourdataset{} is a large-scale indoor synthetic dataset with hybrid motions for point cloud registration, containing diverse movable and deformable foreground objects; and (ii) \ourmethod{} is designed to estimate uncertainty mask for enhancing discriminative feature extraction and accurate correspondence matching against hybrid motions.
    }
    \label{fig: pipeline}
\end{figure*}

==> figures/tex/qualitative_DeforMatch_3DMatch.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pdf/qualitative_DeforMatch_3DMatch.pdf}
    \caption{Qualitative comparison on \ourdataset{} and 3DMatch.}
    \label{fig: qualitative_DeforMatch_3DMatch}
\end{figure*}

==> figures/tex/qualitative_ETH.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pdf/qualitative_ETH.pdf}
    \caption{Qualitative comparison on ETH.}
    \label{fig: qualitative_ETH}
\end{figure}

==> figures/tex/qualitative_corr_mask.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pdf/qualitative_corr_mask.pdf}
    \caption{Visualization of correspondences and uncertainty masks, where unreliable non-rigid regions are marked in red.}
    \label{fig: qualitative_corr_mask}
\end{figure}

==> figures/tex/teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.995\linewidth]{figures/pdf/teaser.pdf}
    \caption{
    We build \ourdataset{}, the first large-scale indoor synthetic dataset with hybrid motions for 3D point cloud registration (top).
    % 
    To improve the robustness, we further design \ourmethod{}, integrating probabilistic uncertainty masks into correspondence estimation (middle), achieving significant boosts (below) in challenging hybrid-motion scenes.
    % 
    }
    \label{fig: teaser}
\end{figure}

==> sections/sec0_abstract.tex <==
% \input{figures/tex/teaser}
\begin{abstract}
Scene-level point cloud registration is very challenging when considering dynamic foregrounds.
% 
Existing indoor datasets mostly assume rigid motions, so the trained models cannot robustly handle scenes with non-rigid motions. 
% 
On the other hand, non-rigid datasets are mainly object-level, so the trained models cannot generalize well to complex scenes. 
% 
This paper presents \ourmethod{}, a new approach to 3D point cloud registration, learning uncertainty mask to account for hybrid motions: rigid for backgrounds and non-rigid/rigid for instance-level foregrounds. 
% 
First, we build a scene-level 3D registration dataset, namely \ourdataset{}, designed specifically with strategies to arrange diverse deforming foregrounds in a controllable manner. 
% 
Second, we account for different motion types and formulate a mask-learning module to alleviate the interference of deforming outliers. 
% 
Third, we exploit a simple yet effective negative log-likelihood loss to adopt uncertainty to guide the feature extraction and correlation computation. 
% 
To our best knowledge, \ourmethod{} is the first work that exploits hybrid motions for robust point cloud registration. 
% 
Extensive experiments show \ourmethod{}'s strengths, leading it to achieve state-of-the-art performance on both widely-used indoor and outdoor datasets. 
% 
Code and dataset will be released to facilitate future research.
%
\end{abstract}

\input{figures/tex/teaser}

==> sections/sec1_intro.tex <==
\section{Introduction}

3D point cloud registration is vital for diverse applications,~\eg, robotics~\cite{elbaz20173d, lu2019l3, li2020deep}, graphics~\cite{zhu2022semi}, vision~\cite{deschaud2018imls, han2019real},~\etc., attracting incredible attention from industry and academia. 
% 
Recent data-driven methods have shown remarkable success, particularly in indoor scenes~\cite{bai2020d3feat, choy2019fully, deng2018ppfnet, huang2020predator, yu2021cofinet, yew2022regtr}, thanks to large-scale datasets like 3DMatch~\cite{zeng20173dmatch}, SIRA-PCR~\cite{Chen_2023_ICCV}, and PointRegGPT~\cite{chen2024pointreggpt}.
%

Typically, the input pair of point clouds are partially overlapping, with 
%
(i) rigid background motions due to the camera motion, and 
(ii) non-rigid foreground motion due to moving or deforming objects.
% 
To align the background, algorithms should eliminate the foreground interference and determine a 3D rigid transformation.
%
However, most existing indoor datasets assume rigid motions in the whole scene, {\em neglecting\/} common non-rigid foreground motions.
% 
So, the first challenge is the lack of a comprehensive benchmark for model training and evaluation on scenes with hybrid motions.
% 

Though directly training on real-captured datasets can alleviate this issue, data collection is highly time-consuming, and data annotation is expensive and error-prone.
% 
An appealing alternative to overcome the data scarcity is to leverage simulated data,~\eg, Lepard~\cite{lepard2021} introduces 4DMatch, an object-level synthetic dataset for non-rigid point cloud registration. 
% 
Yet, models trained on object-level data have proven to struggle to generalize to complex indoor scenes~\cite{qin2022geometric, huang2020predator}, as objects are simpler and have strong shape priors compared to diverse indoor structures.
% 
To sum up, the second challenge is how to design a scene-level benchmark for 3D point cloud registration with hybrid motions, to efficiently account for both data collection and annotations.
% 

Further, even with such appropriate data, algorithms still need to handle outliers in non-overlapping regions, caused not only by different captured views but also by the dynamic foregrounds.
% 
While powerful feature descriptors help address the former, they lack specific designs to handle the latter, as points from foreground objects with similar local geometric structures may be outliers due to inconsistent motions with the background. 
%
Directly applying prior methods to hybrid-motion scenes without any technical improvement can lead to heavy performance degradation.
% 
Hence, the third challenge is how to integrate feature extraction and correspondence matching with precise guidance to account for different types of motions.
% 

% In this work, to address the first two challenges, inspired by FlowNet~\cite{dosovitskiy2015flownet} and SIRA-PCR~\cite{Chen_2023_ICCV}, we build the first large-scale indoor synthetic dataset with hybrid motions, named \ourdataset{}. 
% % 
% Specifically, apart from rigid backgrounds provided by 3D-FRONT~\cite{fu20213d}, we simulate non-rigid motions by injecting instance-level rigid motions for objects from ShapeNet~\cite{chang2015shapenet} on the surface of some furniture and in mid-air, hybridized with deforming objects from DeformingThings4D~\cite{li20214dcomplete}. 
% % 

% For challenge (iii), merely training existing models (even the state-of-the-art methods, e.g., PREDATOR~\cite{huang2020predator} or GeoTrans~\cite{qin2022geometric}) on simulated point cloud pairs is insufficient, due to largely increased difficulty in correspondence matching caused by the hybrid motions. Therefore, draw inspiration from the previous 2D motion estimating method PDCNet~\cite{truong2023pdc}, we propose a probabilistic model named \textbf{\ourmethod{}} for learning uncertainty masks to address \textbf{Hybrid} motions in robust 3D point cloud \textbf{Reg}istration.
% % 
% Instead of deterministically predicting the correspondences, the reformulated probabilistic model, in which we not only compute the correspondence relationship but also learn a robust confidence map to model the correspondence-wise uncertainty.
% % 
% Such map indicates the reliability of the correspondence predictions, essential for solving the 3D transformation.
% % 
% To facilitate training, we assume the output follows a Laplace distribution and thus exploit a simple yet effective negative log-likelihood (NLL) loss to integrate the probabilistic uncertainty into the loss, promoting robust correspondence matching.
%

In this work, to address the first two challenges, we draw inspiration from FlowNet~\cite{dosovitskiy2015flownet} and SIRA-PCR~\cite{Chen_2023_ICCV} to create the first large-scale indoor synthetic dataset with hybrid motions, named \ourdataset{}. Specifically, beyond the rigid backgrounds provided by 3D-FRONT~\cite{fu20213d}, we simulate non-rigid motions by applying instance-level rigid motions to objects from ShapeNet~\cite{chang2015shapenet} on the surfaces of some furniture and in mid-air, combined with deforming objects from DeformingThings4D~\cite{li20214dcomplete}.

For the third challenge, training existing models on simulated point cloud pairs proves insufficient due to the increased difficulty in correspondence matching caused by hybrid motions. As shown in Fig.~\ref{fig: teaser}, their performances degrade as the ratio of non-rigid motion increases. To address it, inspired by the 2D motion estimation method~\cite{truong2023pdc}, we propose a probabilistic model named \textbf{\ourmethod{}} to learn uncertainty masks that address \textbf{Hybrid} motions in robust 3D point cloud \textbf{Reg}istration.
Rather than deterministically predicting correspondences, our reformulated probabilistic model computes the correspondence relationships while simultaneously learning a robust confidence map to model correspondence-wise uncertainty. This map indicates the reliability of the correspondence predictions, which is crucial for accurately solving the 3D transformation. To facilitate training, we assume the output follows a Laplace distribution and employ a simple yet effective negative log-likelihood (NLL) loss to incorporate probabilistic uncertainty into the loss function, enhancing robust correspondence matching. Our main contributions are three-fold:
\begin{itemize}
\item
We construct \ourdataset{}, the first large-scale indoor synthetic dataset with hybrid and diverse motions for 3D point cloud registration. 
%
\item
We design \ourmethod{}, a probabilistic model to learn uncertainty masks, guided by an effective negative log-likelihood loss, to account for hybrid motions and enhance feature extraction and correspondence matching.
%against.  
%
\item
Extensive qualitative and quantitative comparisons on both widely-used indoor and outdoor datasets demonstrate the state-of-the-art performance of our approach.
\end{itemize}

==> sections/sec2_rw.tex <==
\section{Related Work}
\paragraph{Rigid 3D point cloud registration.}
% aims to estimate a 3D rigid transformation to align the input point cloud pair. 
% 
Most approaches are correspondence-based, evolved from traditional handcrafted features~\cite{besl1992method, rusinkiewicz-normal-sampling, segal2009generalized, yang2013go, rusinkiewicz2019symmetric, FPFH} and RANSAC~\cite{fischler1981random} to deep-learning-based feature descriptors~\cite{choy2019fully, gojcic2019perfect, bai2020d3feat, ao2021spinnet, poiesi2022learning, wang2022you, yu2021cofinet, yew2022regtr, wang2023roreg, yangone, lepard2021, Ao_2023_CVPR, yu2023peal,  Mei_2023_CVPR, Liu_2023_ICCV, Chen_2023_ICCV, liu2023regformer}, including weighted SVD for efficient transformation derivation~\cite{wang2019deep, wang2019prnet, idam, yew2020-RPMNet, fu2021robust} and deep robust estimators for transformation accuracy~\cite{bai2021pointdsc, choy2020deep, pais20203dregnet, Jiang_2023_CVPR, Zhang_2023_CVPR, Hatem_2023_ICCV}. 
% 
Others are correspondence-free, directly regressing transformations,~\eg,~\cite{aoki2019pointnetlk, xu2021omnet, xu2022finet}, yet they struggle with scalability and generalization when handling complex scenes~\cite{qin2022geometric}.
% 
Existing methods are mainly designed for (i) indoor scenarios, such as 3DMatch~\cite{zeng20173dmatch}, 7Scenes~\cite{shotton2013scene}, SIRA-PCR~\cite{chen2023sira}, and PointRegGPR~\cite{chen2024pointreggpt}, or (ii) object-level scenarios,~\eg, ModelNet40~\cite{chang2015shapenet}, Stanford 3D Scan~\cite{curless1996volumetric}, and AutoSynth~\cite{Dang_2023_ICCV}. 
% 
% All of them, however, consider only rigid motions, ignoring the commonly existing non-rigid motions in practice, \eg, moving humans/objects.
% 
In this work, we create the first large-scale indoor synthetic dataset with hybrid motions, enabling training and testing to effectively account for deformable foregrounds.
% 

\input{figures/tex/pipeline}

\vspace*{-1mm}
\paragraph{Non-rigid correspondence estimation} is a major topic in dynamic reconstruction~\cite{bozic2020deepdeform, gao18surfelwarp, innmann2016volumedeform, newcombe2015dynamicfusion} and geometry processing~\cite{huang2008non, groueix20183d, ovsjanikov2012functional, attaiki2023understanding, rodola2017partial}, focusing on estimating non-rigid correspondences from deformable point clouds or manifold surfaces.
% 
DynamicFusion~\cite{newcombe2015dynamicfusion} employs 
%simple 
projective correspondence for real-time efficiency and is further utilized for dense correspondence learning in~\cite{schmidt2016self}.
% 
VolumeDeform~\cite{innmann2016volumedeform} adopts SIFT~\cite{lowe2004distinctive} for robust non-rigid tracking. 
% 
DeepDeform~\cite{bozic2020deepdeform} learns sparse global correspondence for patches in deforming RGB-D sequences. 
% 
\cite{li2020learning} learn non-rigid features via a differentiable non-rigid alignment optimization. 
% 
%NNRT~\cite{bozic2020neural} focuses on end-to-end correspondence estimation with an outlier rejection network. 
NNRT~\cite{bozic2020neural} estimate correspondence end-to-end with an outlier rejection network. 
% 
Besides, scene flow estimation,~\eg,~\cite{li2021neural, dosovitskiy2015flownet, liu2019flownet3d, puy2020flot, wu2020pointpwc}, is a closely-related technique that delivers point-wise correspondence.
% 
The key difference between our task and these works is that non-rigid correspondences on moving or deforming foreground objects are outliers and should be filtered out for accurate background alignment in our scene-level task.


==> sections/sec3_method.tex <==
\section{Method}

\subsection{Overview}
Fig.~\ref{fig: pipeline} gives an overview of our approach, which includes
% 
(i) \ourdataset{}, a large-scale indoor synthetic dataset with hybrid motions for 3D point cloud registration (Sec.~\ref{sec: 3.2});
(ii) \ourmethod{}, the method we designed to estimate probabilistic uncertainty masks and evaluate reliability and accuracy of the correspondence prediction against hybrid motions (Sec.~\ref{sec: 3.3}); and
(iii) our loss function design (Sec.~\ref{sec: 3.4}).
%
%\phil{Perhaps too hard-sell: don't keep saying the first this and that...}
%We construct the first large-scale indoor synthetic dataset with hybrid motions, \ourdataset{}, for 3D point cloud registration (Sec.~\ref{sec: 3.2}).
% 
%Then, we design \ourmethod{} to estimate probabilistic uncertainty masks, indicating the reliability and accuracy of the correspondence prediction against hybrid motions, which is indispensable for the registration task (Sec.~\ref{sec: 3.3}).
% 
%Finally, loss functions are presented in Sec.~\ref{sec: 3.4}.
% 

\subsection{\ourdataset{} Dataset} 
\label{sec: 3.2}
Existing indoor datasets typically contain only static scenes, yet dynamic scenes are common in the real world. To better simulate real-world environments, our \ourdataset{} includes not only rigid background motions but also a diverse range of rigid and non-rigid foreground motions for objects within the background scene, such as humans moving around, animals wandering, and objects or furniture shifting. This makes \ourdataset{} more representative of the complexities found in everyday indoor environments.
% 
To achieve this level of realism, we carefully design different strategies for various types of motion.
% 

\paragraph{Rigid scene-level background motions.}
We construct the indoor scene background using 3D-FRONT, as it offers professionally-designed room layouts and a rich variety of furniture.
% 
To enhance the scene complexity, following~\cite{chen2023sira}, models from the ShapeNet dataset are randomly scaled, rotated, and placed either mid-air in the rooms or on existing furniture items such as tables and beds.
% 
The rigid background motion is naturally introduced when adjusting the camera view in the point cloud rendering process.
% 

\paragraph{Non-rigid/rigid object-level foreground motions.}
Given a room layout, we consider two distinct cases of injecting foreground object motions based on the rigidity of the object:
% 
(i) Deformable non-rigid objects, such as humans and animals. 
% 
Inspired by~\cite{lepard2021}, we employ models and offsets from the DeformingThings4D dataset, a synthetic collection, comprising thousands of animation sequences across various categories of humanoids and animals. 
% 
For each scene, animation sequences are randomly selected; half feature a single human and the other half feature multiple humans and animals.
% 
To enhance the diversity in movement magnitude, we employ random offsets to the human and animal models in every frame.
% 
(ii) Movable rigid objects, such as chairs and cups. 
% 
First, additional rigid models from ShapeNet are positioned around each deformable non-rigid object in (i), with random XY-plane offsets applied to each frame to simulate movement and introduce noise.
% 
To augment realism, we introduce subtle movements to movable furniture items, thereby enriching the scene's plausibility with hybrid motions.
% 
Care is taken to ensure that each foreground object insertion is collision-free, maintaining the physical plausibility of the scene.
% 

\paragraph{Registration data preparation.}
To produce paired data for point cloud registration, we follow~\cite{chen2023sira} to use a virtual perspective camera to render a depth map for each viewpoint, subsequently converting these maps into point clouds. 
% 
% The camera height is set at 1.6m to simulate human visual experience. 
% 
We limit the depth range and randomly remove half of the large flat surfaces, such as walls and floors, to emphasize the foreground. 
% 
% Additional noise is introduced to closely replicate real-world conditions.
% 
To ensure scene complexity, high-quality camera views are selected. 
% 
The viewing range is set to [0\textdegree,360\textdegree] horizontally and [0\textdegree,45\textdegree] vertically, with views uniformly sampled at intervals of 30\textdegree and 15\textdegree, respectively.
% 
Ground-truth correspondences of the overlapping point cloud pairs are easily established, given the accurate camera poses. 
% 
Following 3DMatch, we categorize our data into \ourdataset{} ($<$30\% overlap ratio) and \ourlodataset{} (10-30\% overlap ratio).
% 
Based on the proportion of non-rigid motions, each set is further divided into \emph{10-30\% non-rigid} and \emph{30-50\% non-rigid} splits.
% 
To validate our data, each pair is accompanied by a corresponding pair without any animations, forming a \emph{rigid-only} split.
% 
For each split, we create a validation/test set, consisting of 100/1,000 pairs.
% 

\subsection{\ourmethod{}} 
\label{sec: 3.3}
\paragraph{Problem formulation.}
% 
Given the input point cloud pair $\mathcal{I} = (\mathcal{P}, \mathcal{Q})$, where 
%$\mathcal{P} \!\in\! \mathbb{R}^{N \times 3}, \mathcal{Q} \!\in\! \mathbb{R}^{M \times 3}$ are source and target point clouds with $N$ and $M$ points, respectively,
$\mathcal{P} \!\in\! \mathbb{R}^{N \times 3}$ is the source point point with $N$ points and 
$\mathcal{Q} \!\in\! \mathbb{R}^{M \times 3}$ is the target with $M$ points.
% 
A network $F$ with parameters $\theta$ is employed to estimate the correspondences $\mathcal{C}$, \ie, $\mathcal{C} \!=\! F(\mathcal{I};\theta)$. 
% 
Then, the 3D transformation $\{\mathbf{R}\!\in\! S O(3),\mathbf{t} \!\in\! \mathbb{R}^3\}$ is derived from $\mathcal{C}$.

\paragraph{Feature extraction.}
We first downsample the source and target points to obtain superpoints $\hat{\mathcal{P}}$ and $\hat{\mathrm{Q}}$ as in~\cite{qin2022geometric}. 
% 
% Here we use $\hat{N}$ and $\hat{M}$ to denotes the number of source and target superpoints, respectively. 
% 
Utilizing KPConv-FPN~\cite{thomas2019kpconv}, we extract features of the point clouds, with the associated learned features denoted as $\mathbf{F}^{\hat{\mathcal{P}}} \!\in\! \mathbb{R}^{\hat{N} \times d}$ and $\mathbf{F}^{\hat{\mathcal{Q}}} \!\in\! \mathbb{R}^{\hat{M} \times d}$. 
% 

\paragraph{Geometric transformer.}
Following~\cite{qin2022geometric}, we employ geometric self-attention mechanisms to learn global correlations among superpoints within each point cloud. 
% 
Here, we describe the computation for $\hat{\mathcal{P}}$, and the same process applies to $\hat{\mathcal{Q}}$. 
% 
Given the input feature matrix $\mathbf{X} \!\in\! \mathbb{R}^{\hat{N}\times{d_t}}$, the self-attention feature $\mathbf{Z} \!\in\! \mathbb{R}^{\hat{N}\times{d_t}}$ is computed as the cumulative weighted sum of all projected input features: 
% 
$\mathbf{Z}_i\!=\!\sum\nolimits_{j=1}^{\hat{N}}a_{i,j}({\mathbf{X}_j}\mathbf{W}^V)$,
% 
where the weight coefficient $a_{i,j}\!=\!\operatorname{Softmax}(\frac{(\mathbf{X}_i\mathbf{W}^Q)(\mathbf{X}_j\mathbf{W}^K +\mathbf{R}_{i,j}\mathbf{W}^R)^T}{\sqrt{d_t}})$. 
% 
$\mathbf{R}_{i,j} \!\in\! \mathbb{R}^{d_t}$ represents the geometric structure embedding, which includes pairwise distances and angular information among points.
% 
$\mathbf{W}$ denotes the projection matrix, whose superscripts $Q$, $K$, $V$, and $R$ correspond to queries, keys, values, and geometric structure embeddings, respectively.
% 
Then, to encode inter-frame geometric consistency, cross-attention mechanisms are adopted.
% 
The cross-attention feature $\mathbf{Z}^{\hat{\mathcal{P}}} \!\in\! \mathbb{R}^{\hat{N}\times{d_t}}$ for $\hat{\mathcal{P}}$ is computed as 
$\mathbf{Z}_i^{\hat{\mathcal{P}}}\!=\!\sum\nolimits_{j=1}^{\hat{M}}a_{i,j}({\mathbf{X}_j^{\hat{\mathcal{Q}}}}\mathbf{W}^V)$,
% 
where the weight coefficient $a_{i,j}\!=\!\operatorname{Softmax}(\frac{(\mathbf{X}_i^{\hat{\mathcal{P}}}\mathbf{W}^Q)(\mathbf{X}_j^{\hat{\mathcal{Q}}}\mathbf{W}^K)^T}{\sqrt{d_t}})$.
% 

\paragraph{Uncertainty mask generation.}
% 
Previous methods typically predict correspondences $\mathcal{C}$ directly by $\mathcal{C} \!=\!\! F(\mathcal{I}; \theta)$, however, it does not provide confidence measures.
% 
Instead, our objective is to estimate the conditional probability density function $p(\mathcal{C} | \mathcal{I};\theta)$, which allows us to capture the uncertainty associated with the predictions. 
% 
To achieve this, we design a network to predict the parameters $\Phi(\mathcal{I};\theta)$ of a family of distributions, \ie,
\begin{equation}
    p(\mathcal{C} | \mathcal{I};\theta)=p(\mathcal{C} | \Phi(\mathcal{I};\theta))=\Pi_{i,j}p(c_{i,j} | \varphi_{i,j}(\mathcal{C;\theta})).
\end{equation}
% 
For tractable estimation, we assume conditional independence between the predictions for the $i$-th source point and the $j$-th target point.
% 
Here, $c_{i,j} \!\in\! \{0,1\}$ is the ground-truth correspondence relationship, and $\varphi_{i,j} \!\in\! \mathbb{R}^n$ denotes the predicted parameters, including both the predicted correspondence relationship and the confidence. 
% 
For simplicity, we omit the subscript $i,j$ in the subsequent discussion.
% 

Compared to the direct prediction approach $\mathcal{C} \!=\! F(\mathcal{I}; \theta)$, the parameters $\Phi(\mathcal{I}; \theta)$ of the predictive distribution encode additional information about the correspondence, including its uncertainty. 
% 
Following previous works~\cite{ilg2018uncertainty, kendall2017uncertainties, truong2023pdc}, this is done by predicting the variance of the correspondence. 
% 
In these cases, the predictive density $p(c|\varphi)$ is modeled using Laplace distributions:
\begin{equation}
\label{eq: laplace}
    \mathcal{L}(c|\sigma^2)=\frac{1}{\sqrt{2 \sigma^2}} e^{-\sqrt{\frac{2}{\sigma^2}}|c-\mu|} ,
\end{equation}
where the mean $\mu$ and variance $\sigma^2$ are predicted by the network as $(\mu,\sigma^2)=\Phi(\mathcal{I};\theta)$ for each point pair. $\sigma^2$ serves as the uncertainty mask, indicating higher confidence for matching pairs likely to overlap and lower confidence for non-overlapping or foreground regions. 
%

To predict the uncertainty mask, we first compute the cross-attention feature $\mathbf{G}^{\hat{\mathcal{P}}} \!\in\! \mathbb{R}^{\hat{N}\times{d_t}}$ for $\hat{\mathcal{P}}$ after obtaining the self-attention features $\mathbf{H}^{\hat{\mathcal{P}}}$ and $\mathbf{H}^{\hat{\mathcal{Q}}}$, \ie,
% 
\begin{equation}
    \mathbf{G}_i^{\hat{\mathcal{P}}}\!=\!\sum\nolimits_{j=1}^{\hat{M}}a_{i,j}({\mathbf{H}_j^{\hat{\mathcal{Q}}}}\mathbf{W}^V),
\end{equation}
% 
where $a_{i,j}\!=\!\operatorname{Softmax}(\frac{(\mathbf{H}_i^{\hat{\mathcal{P}}}\mathbf{W}^Q)(\mathbf{H}_j^{\hat{\mathcal{Q}}}\mathbf{W}^K)^T}{\sqrt{d_t}})$
%
is the weight coefficient computed by applying a row-wise softmax on the cross-attention score. Similarly, we can derive the cross-attention feature $\mathbf{G}^{\hat{\mathcal{Q}}}$ for $\mathcal{Q}$. 
% 
$\mathbf{G}^{\hat{\mathcal{P}}}$ and $\mathbf{G}^{\hat{\mathcal{Q}}}$ exhibit robust geometric characteristics and awareness of hybrid motions between the input point clouds. 
% 
Finally, we use an MLP, $\Phi$ with parameters $\theta$ followed by a sigmoid layer, to regress the uncertainty masks, \ie,
% 
$\sigma^2_{\hat{\mathcal{P}}},\sigma^2_{\hat{\mathcal{Q}}}= \operatorname{Sigmoid}(\Phi(\mathbf{G}^{\hat{\mathcal{P}}}, \mathbf{G}^{\hat{\mathcal{Q}}};\theta)).$
% 

\paragraph{Uncertainty-aware superpoint matching.}
To determine superpoint correspondences, we follow \cite{qin2022geometric} to first normalize $\mathbf{H}^{\hat{\mathcal{P}}}$ and $\mathbf{H}^{\hat{\mathcal{Q}}}$ onto a unit hypersphere.
% 
Then, we compute the Gaussian correlation matrix $\mathbf{S} \!\in\! \mathbb{R}^{\hat{N}\times\hat{M}}$, where $s_{i,j}=\operatorname{exp}(-||\mathbf{h}_i^{\hat{\mathcal{P}}}-\mathbf{h}_i^{\hat{\mathcal{Q}}}||_2^2)$. 
% 
Besides, a dual-normalization operation~\cite{rocco2018neighbourhood, sun2021loftr} is performed on $\mathbf{S}$ to suppress ambiguous matches.
% 
To further enhance the robustness against incorrect matches caused by hybrid motions, we mask the correlation matrix $\mathbf{S}$ using our generated uncertainty masks. We then select the largest $N_c$ entries as the superpoint correspondences, \ie,
\begin{equation}
    \hat{\mathcal{C}}=\{(\hat{\mathbf{p}}_{x_i},\hat{\mathbf{q}}_{y_i})|(x_i,y_i)\in\operatorname{topk}_{x,y}(s_{x,y}\cdot \sigma^2_{x,y})\},
\end{equation}
where $\hat{\mathbf{p}}_{x_i}$ and $\hat{\mathbf{q}}_{y_i}$ are superpoints in $\hat{\mathcal{P}}$ and $\hat{\mathcal{Q}}$, respectively.
% 

\paragraph{Transformation estimation.} 
To recover the 3D transformation between the inputs based on the estimated correspondences, we employ both the RANSAC algorithm and the deep robust estimator LGR proposed by~\cite{qin2022geometric}.
% While RANSAC is known for its robustness, it often suffers from slow convergence. 
% 
% Conversely, LGR achieves faster and more accurate registration by first generating 3D transformation candidates from local patch pairs through weighted SVD and then validate them across all correspondences to select the optimal transformation.

\input{tables/DeforMatch_LGR}
\input{tables/DeforMatch_RANSAC}


\subsection{Loss Functions} 
\label{sec: 3.4}
The loss function consists of an uncertainty mask loss $\mathcal{L}_{um}$ for uncertainty prediction, an overlap-aware circle loss $\mathcal{L}_{oc}$ for superpoint matching, and a point matching loss $\mathcal{L}_{p}$.  
% 
Both $\mathcal{L}_{oc}$ and $\mathcal{L}_{p}$ are implemented following~\cite{qin2022geometric}. 
% 
The overall loss for training is $\mathcal{L}=\mathcal{L}_{um}+\mathcal{L}_{oc}+\mathcal{L}_{p}$.
% 
%\phil{TODO: shorten the above paragraph? No need to repeat the names of each loss}

\paragraph{Uncertainty mask loss $\mathcal{L}_{um}$.}
As customary in probabilistic regression~\cite{ilg2018uncertainty, kendall2017uncertainties, truong2023pdc}, we employ the negative log-likelihood loss to train the uncertainty mask generator:
\begin{equation}
    -\log p(\mathcal{C}|\Phi(\mathcal{I};\theta)\!=\!-\!\sum\nolimits_{i,j}\log p(c_{i,j}|\varphi_{i,j}(\mathcal{I};\theta)),
\end{equation}
where $p(c|\varphi)$ can be substituted by the Laplace distribution as detailed in Eq.~\ref{eq: laplace}. Taking into account both source and target uncertainty masks, $\mathcal{L}_{um}$ is formulated as
\begin{equation}
    \mathcal{L}_{um}\!=\!-\log(\sum\nolimits_{i,j}\!e^{\scriptscriptstyle{-\log(2)-\alpha_{i,j}-\sqrt{2}e^{-\frac{1}{2}\alpha_{i,j}}\cdot |c_{i,j}-\mu_{i,j}|}}),
\end{equation}
where $\alpha_{i,j} \!=\! \log(\sigma^2_{\hat{\mathcal{P}}} \!\cdot\! \sigma^2_{\hat{\mathcal{Q}}})_{i,j}$. 
% 
Naturally, we use $\mu_{i,j} \!=\! s_{i,j}$ in the Gaussian correlation matrix $\mathbf{S}$ to denote the correspondence prediction for the point pair $i,j$.
% 
To avoid division by zero, we use a numerically stable log-sum-exp function and introduce a regularization term $1-\sigma^2_{\hat{\mathcal{P}}} \!\cdot\! \sigma^2_{\hat{\mathcal{Q}}}$.
% 

\paragraph{Overlap-aware circle loss $\mathcal{L}_{oc}$.}
To prioritize matches with high overlap, we compute the overlap-aware circle loss on $\mathcal{P}$,
\begin{equation}
    \mathcal{L}_{oc}^{\mathcal{P}} \! = \! \frac{1}{|\mathcal{A}|}  \!\!  \sum_{\mathcal{G}^{\mathcal{P}}_i \in \mathcal{A}} \!\!\! \log[1 + \! \! \! \sum_{\mathcal{G}^{\mathcal{Q}}_j \in \varepsilon_p^i} \!\!\!\!  e^{\lambda_i^j \beta_p^{i,j}(d_i^j - \Delta_p)} \cdot \!\!\!\! \sum_{\mathcal{P}^{\mathcal{Q}}_k\in \varepsilon_n^i} \!\!\!\! e^{\beta_p^{i,k}(\Delta_n - d_i^k)}].
\end{equation}
Here, $\mathcal{A}$ is the set of anchor patches in $\mathcal{P}$ that have at least one positive patch in $\mathcal{Q}$. 
%
For each anchor patch $\mathcal{G}^{\mathcal{P}}_i \! \in \! \mathcal{A}$, $\varepsilon_p^i$ and $\varepsilon_n^i$ denote the sets of its positive and negative patches in $\mathcal{Q}$. 
%
$d_i^j$ is the feature distance, and $\lambda_i^j = (o_i^j)^{\frac{1}{2}}$ and $o_i^j$ represents the overlap ratio between $\mathcal{G}^{\mathcal{P}}_i$ and $\mathcal{G}^{\mathcal{Q}}_j$. 
%
$\beta_p^{i,j} \!=\! \gamma(d_i^j \!-\! \Delta_p)$ and $\beta_n^{i,k} \!=\! \gamma(\Delta_n \!-\! d_i^k)$ are the positive and negative weights, respectively. 
%
The margins $\Delta_p$ and $\Delta_n$ are set to 0.1 and 0.4, respectively. The same goes for the loss $\mathcal{L}_{oc}^{\mathcal{Q}}$ on $\mathcal{Q}$.
% 


\paragraph{Point matching loss $\mathcal{L}_{p}$}
is computed for the $i$th patch as
\begin{equation}
    \mathcal{L}_{p,i} = - \! \! \! \! \! \! \! \sum_{(u,v) \in \mathcal{M}_i} \! \! \! \! \! \! \log \Bar{z}_{\scriptscriptstyle{u,v}}^i - \! \! \! \sum_{u \in \mathcal{I}_i} \log \Bar{z}_{\scriptscriptstyle{u,m_i+\!1}}^i - \! \! \! \sum_{v \in \mathcal{J}_i} \log \Bar{z}_{\scriptscriptstyle{n_i+\!1, v}}^i,
\end{equation}
where $\mathcal{M}_i$ denotes the set of ground-truth point correspondences extracted with a matching radius $\tau$ from each $\hat{\mathcal{C}}_i^*$ and $\{ \hat{\mathcal{C}}_i^* \}$ denotes the randomly sampled $N_g$ ground-truth point correspondences. $\Bar{z}_{u,v}^i$ is the element in the $u$-th row and the $v$-th column of the soft assignment matrix $\Bar{\mathbf{Z}}_i$. $\mathcal{I}_i$ and $\mathcal{J}_i$ denote the sets of unmatched points in the two patches.



==> sections/sec4_exp.tex <==
\section{Experiments}


\input{figures/tex/qualitative_DeforMatch_3DMatch}
\input{tables/3DMatch}


\subsection{Datasets and Evaluation Metrics}
\paragraph{Datasets.}
To evaluate effectiveness on hybrid motions, we use the proposed \ourdataset{}/\ourlodataset{}, which is divided into three splits: \emph{rigid-only} (11.3k/14k pairs), \emph{10-30\% non-rigid} (7.3k/8.5k pairs), and \emph{30-50\% non-rigid} (4k/5.5k pairs). 
% 
To assess robustness in indoor scenes, we employ the 3DMatch dataset~\cite{zeng20173dmatch}, comprising 62 scenes, with 46/8/8 scenes used for training, validation, and testing, respectively. 3DMatch and 3DLoMatch are categorized based on $<$30\% and 10\%-30\% overlap ratios. 
% 
To evaluate {the} generalizability in outdoor scenes, we use the ETH dataset~\cite{pomerleau2012challenging}, including 4 scenes with 713 pairs of 132 point clouds.
% 
% It is particularly challenging due to luxuriant trees and small structures. 
% 
Evaluations on ETH use models trained on 3DMatch.
% 

\paragraph{Evaluation metrics.}
We adopt several metrics following~\cite{qin2022geometric,chen2023sira}: 
% 
(i) Registration Recall (RR), the fraction of successfully registered pairs whose transformation error RMSE$<$0.2m/0.2m/0.5m for \ourdataset{}/3DMatch/ETH; 
% 
(ii) Inlier Ratio (IR), the fraction of inlier correspondences with residuals $<$0.1m/0.1m/0.2m for \ourdataset{}/3DMatch/ETH; 
% 
(iii) Feature Matching Recall (FMR), the fraction of pairs with IR$>$5\%; 
% 
(iv) The median of the average Relative Rotation Error (RRE); and 
% 
(v) The median of the average Relative Translation Error (RTE) for successfully registered pairs whose RMSE$<$0.2m/0.2m/0.5m for \ourdataset{}/3DMatch/ETH.
% 


\subsection{Implementation Details}
% The rendering settings of our \ourdataset{} are similar to those of SIRA-PCR~\cite{chen2023sira}, and the hyperparameters are set similarly to those in GeoTrans~\cite{qin2022geometric}.
% 
To stabilize the training, we adopt a two-stage strategy. 
% 
The batch size is set to be 8. The uncertainty mask generator is first trained with L1 loss for 30 epochs, then fine-tuned with uncertainty mask loss for 20 epochs. 
% 
Adam optimizer~\cite{kingma2014adam} is used for training with a batch size of one and a learning rate of 1e-4.
% 
All experiments are conducted on 8 NVIDIA Tesla P40 GPUs.
% 
Please refer to our supp. material for more details.


\input{figures/tex/qualitative_corr_mask}


\subsection{Evaluation on \ourdataset{}}
We compare the quantitative registration results of our method with recent state-of-the-art approaches in Tab.~\ref{tab: DeforMatch_LGR} and Tab.~\ref{tab: DeforMatch_RANSAC}. 
% 
As revealed in Tab.~\ref{tab: DeforMatch_LGR}, either transferring pre-trained model weights from 3DMatch to our \ourdataset{} \emph{rigid-only} split or direct training on our data yields high RR, validating our synthetic data.
%
However, models trained on rigid-only data struggle with hybrid motions, particularly in scenarios with significant foreground motion and low overlap.
% 
Incorporating hybrid-motion data into training improves performance but remains inferior to rigid-only scenes, highlighting the need for algorithmic enhancements.
% 
Our \ourmethod{} significantly outperforms other methods across almost all metrics, demonstrating robust registration capability for both rigid-only and challenging non-rigid scenarios. 
% 
Specifically, our method achieves a 20.7\% increase in RR compared to the second best on the most challenging test split (\ourlodataset{}, \emph{30-50\% non-rigid}). 
% 
Qualitative results in Fig.~\ref{fig: qualitative_DeforMatch_3DMatch} also illustrate our method's superior performance.
% 
We visualize our uncertainty masks in Fig.~\ref{fig: qualitative_corr_mask}, where the precise masks improve the correspondence accuracy.


\input{tables/ablation_DeforMatch_HybridReg}
\input{tables/ETH}


\subsection{Evaluation on Rigid Benchmark}
\paragraph{Evaluation on indoor 3D(Lo)Match.}
Results on the rigid-only 3DMatch dataset are presented in Tab.~\ref{tab: 3DMatch}.
% 
Our \ourmethod{} achieves state-of-the-art performance on 3DMatch and competitive results on 3DLoMatch, highlighting its ability to preserve the strength on rigid-only scenes effectively.
% 
Fig.~\ref{fig: qualitative_DeforMatch_3DMatch} also indicates the effectiveness of our method. 
% 


\paragraph{Evaluation on outdoor ETH.}
To assess generalizability, we transfer models trained on 3DMatch to the ETH dataset, following~\cite{wang2023roreg, chen2023sira}. 
% 
As shown in Tab.~\ref{tab: ETH}, our method outperforms the baseline (GeoTrans) and most other methods in RR, showcasing strong generalization capability in outdoor scenes. 
% 
The qualitative comparison in Fig.~\ref{fig: qualitative_ETH} shows our method's effectiveness in addressing challenging cases with complex, unseen structures.
% 

\subsection{Ablation Study}
We conduct extensive experiments on our \ourdataset{} and \ourmethod{} to evaluate the impact of each component. 
% 
The hybrid-motion test set is fixed for consistent evaluation.
% 


\paragraph{\ourdataset{}.}
We detail the construction of our \ourdataset{} in Tab.~\ref{tab: ablation_DeforMatch_HybridReg} (a-d).
% 
By incrementally incorporating components into our baseline, we assess their contributions to the model's performance on the test set.
% 
Comparing Rows (a) and (b), injecting non-rigid motions from DeformingThings4D significantly boosts registration performance.
% 
Rows (c-d) and (b) demonstrate that adding rigid motions to selected foreground objects (c) and removing planes to balance geometric structures (d) help the model focus on background motion, thereby improving performance.
% 


\input{figures/tex/qualitative_ETH}



\paragraph{\ourmethod{}.}
To understand the efficacy of components in \ourmethod{}, we ablate each of them as shown in Tab.~\ref{tab: ablation_DeforMatch_HybridReg} (e-h).
% 
Initially, we integrate the uncertainty mask learning module into the baseline, employing two loss variants for supervision.
% 
Comparing Rows (f-g) and (e), the negative log-likelihood (NLL) loss outperforms the L1 loss in enhancing uncertainty modeling and learning capabilities, leading the model to better identify inlier correspondences, such as rigid background and immovable foreground. 
% 
Further, comparing Rows (g) and (h), using the predicted uncertainty mask to refine the Gaussian correlation matrix yields an additional performance boost by suppressing incorrect matches.
% 


==> sections/sec5_conclusion.tex <==
\section{Conclusion}
We introduce \ourmethod{}, a novel 3D point cloud registration framework to account for hybrid motions and to enhance robustness.
% 
To our best knowledge, we create the first large-scale indoor synthetic dataset, \ourdataset{}, tailored for point cloud registration with hybrid motions.
% 
Also, we propose a probabilistic uncertainty mask-learning module to mitigate the impact of deforming outliers. 
% 
Experimental results manifest the SOTA performance of \ourmethod{} consistently on various indoor and outdoor benchmarks.
% 
We will release our code and model weights as open source.

==> tables/3DMatch.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|ccc|ccc}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{3DMatch} & \multicolumn{3}{c}{3DLoMatch} \\
        \cmidrule{2-7}
        & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ \\
        \midrule
        PerfectMatch & 2.2 & 7.1 & 78.4 & 3.5 & 10.3 & 33.0 \\
        FCGF & \underline{2.0} & 6.6 & 85.1 & 3.2 & 10.0 & 40.1  \\
        D3Feat & 2.2 & 6.7 & 81.6 & 3.4 & 10.3 & 37.3 \\
        PREDATOR & \underline{2.0} & 6.4 & 89.0 & 3.1 & 9.3 & 59.8  \\
        CoFiNet & \underline{2.0} & 6.2 & 89.3 & 3.3 & 9.4 & 67.5 \\
        GeoTrans & \textbf{1.6} & 5.3 & 91.5 & \textbf{2.5} & \textbf{7.4} & \textbf{74.0} \\
        RegTR & \textbf{1.6} & \textbf{4.9} & \underline{92.0} & \underline{2.8} & 7.7 & 64.8 \\
        \midrule
        Our \ourmethod{} & \textbf{1.6} & \underline{5.2} & \textbf{92.7} & \textbf{2.5} & \underline{7.5} & \underline{73.1} \\
        \bottomrule
    \end{tabular}}
    \caption{Registration results on 3DMatch and 3DLoMatch.}
    \label{tab: 3DMatch}
    % \vspace{-3mm}
\end{table}

==> tables/DeforMatch_LGR.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Evaluation results on our DeforMatch and DeforLoMatch.}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|ccc|ccc|ccc|ccc}
%         \toprule
%          \multirow{4}{*}{Methods} & \multicolumn{6}{c|}{DeforMatch} & \multicolumn{6}{c}{DeforLoMatch} \\
%          \cmidrule{2-13}
%          & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c|}{\textit{30-50\% non-rigid}} & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c}{\textit{30-50\% non-rigid}}\\
%          \cmidrule{2-13}
%          & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ \\
%          \midrule
%          % D3Feat~\cite{bai2020d3feat} & 3.0 & 19.0 & 20.1 & 3.5 & 22.2 & 24.4 & 3.8 & 19.4 & 3.4 & 3.7 & 21.7 & 5.4 \\
%          % BUFFER~\cite{Ao_2023_CVPR} & 5.2 & 24.1 & 37.4 & 6.2 & 26.4 & 34.2 & 6.4 & 29.9 & 6.6 & 5.9 & 20.3 & 5.4 \\
%          % Lepard~\cite{lepard2021} & 4.6 & 18.8 & 19.6 & 4.4 & 15.8 & 20.2 & 5.2 & 26.8 & 3.6 & 5.1 & 26.4 & 3.2 \\
%          Predator & 4.6 & 19.2 & 31.6 & 5.6 & 24.5 & 26.6 & 9.7 & 34.9 & 6.2 & 8.2 & 30.4 & 5.0 \\
%          CoFiNet & 3.8 & 12.9 & 33.6 & 4.0 & 17.8 & 28.2 & 7.5 & 25.0 & 5.0 & 6.2 & 29.4 & 5.8 \\
%          GeoTrans & 3.7 & 13.6 & 27.6 & 4.0 & 17.6 & 22.6 & 5.7 & 18.3 & 5.2 & 5.7 & 25.5 & 1.4 \\
%          \midrule
%          Predator$^\dagger$ & 2.4 & 8.7 & 80.8 & 2.8 & 12.6 & 75.4 & 5.1 & 17.5 & 33.2 & 4.2 & 17.5 & 24.4 \\
%          CoFiNet$^\dagger$ & 2.8 & 10.6 & 82.4 & 3.3 & 14.6 & 78.0 & 5.1 & 18.0 & 29.8 & 4.7 & 23.1 & 25.6 \\
%          GeoTrans$^\dagger$ & 1.4 & 5.6 & 95.6 & 1.6 & 8.1 & 93.6 & 3.3 & 12.3 & 64.2 & 3.2 & 13.7 & 61.0 \\
%          Our HybridReg & 1.2 & 5.4 & 97.4 & 1.5 & 7.1 & 96.6 & 3.0 & 12.2 & 75.6 & 2.8 & 12.3 & 73.6 \\
%          \bottomrule
%     \end{tabular}}
%     \label{tab:DeforMatch_LGR}
% \end{table*}
\begin{table*}[th]
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
        \toprule
         \multirow{4}{*}{Methods} & \multicolumn{9}{c|}{HybridMatch} & \multicolumn{9}{c}{HybridLoMatch} \\
         \cmidrule{2-19}
         & \multicolumn{3}{c|}{\textit{rigid-only}} & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c|}{\textit{30-50\% non-rigid}} & \multicolumn{3}{c|}{\textit{rigid-only}} & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c}{\textit{30-50\% non-rigid}}\\
         \cmidrule{2-19}
         & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ \\
         \midrule
         % D3Feat~\cite{bai2020d3feat} & 3.0 & 19.0 & 20.1 & 3.5 & 22.2 & 24.4 & 3.8 & 19.4 & 3.4 & 3.7 & 21.7 & 5.4 \\
         % BUFFER~\cite{Ao_2023_CVPR} & 5.2 & 24.1 & 37.4 & 6.2 & 26.4 & 34.2 & 6.4 & 29.9 & 6.6 & 5.9 & 20.3 & 5.4 \\
         % Lepard~\cite{lepard2021} & 4.6 & 18.8 & 19.6 & 4.4 & 15.8 & 20.2 & 5.2 & 26.8 & 3.6 & 5.1 & 26.4 & 3.2 \\
         PREDATOR$^\dagger$ & 1.7 & 6.7 & 98.7 & 4.6 & 19.2 & 31.6 & 5.6 & 24.5 & 26.6 & 2.0 & 7.6 & 89.9 & 9.7 & 34.9 & 6.2 & 8.2 & 30.4 & 5.0 \\
         CoFiNet$^\dagger$ & 1.3 & 5.2 & \underline{99.2} & 3.8 & 12.9 & 33.6 & 4.0 & 17.8 & 28.2 & 1.8 & 7.2 & 93.0 & 7.5 & 25.0 & 5.0 & 6.2 & 29.4 & 5.8 \\
         GeoTrans$^\dagger$ & 0.8 & 3.2 & 98.9 & 3.7 & 13.6 & 27.6 & 4.0 & 17.6 & 22.6 & \underline{1.1} & 4.2 & 91.3 & 5.7 & 18.3 & 5.2 & 5.7 & 25.5 & 1.4 \\
         \midrule
         PREDATOR$^\ddagger$ & 1.1 & 4.4 & 98.9 & 2.4 & 8.7 & 80.8 & 2.8 & 12.6 & 75.4 & 1.4 & 5.3 & \textbf{94.6} & 5.1 & 17.5 & 33.2 & 4.2 & 17.5 & 24.4 \\
         CoFiNet$^\ddagger$ & 1.4 & 5.8 & 98.2 & 2.8 & 10.6 & 82.4 & 3.3 & 14.6 & 78.0 & 1.8 & 7.3 & 88.9 & 5.1 & 18.0 & 29.8 & 4.7 & 23.1 & 25.6 \\
         GeoTrans$^\ddagger$ & \underline{0.6} & \underline{2.3} & \textbf{99.3} & \underline{1.4} & \underline{5.6} & \underline{95.6} & \underline{1.6} & \underline{8.1} & \underline{93.6} & \textbf{0.8} & \underline{3.4} & 93.8 & \underline{3.3} & \underline{12.3} & \underline{64.2} & \underline{3.2} & \underline{13.7} & \underline{61.0} \\
         Our \ourmethod{}$^\ddagger$ & \textbf{0.5} & \textbf{2.1} & \underline{99.2} & \textbf{1.2} & \textbf{5.4} & \textbf{97.4} & \textbf{1.5} & \textbf{7.1} & \textbf{96.6} & \textbf{0.8} & \textbf{3.3} & \underline{93.9} & \textbf{3.0} & \textbf{12.2} & \textbf{75.6} & \textbf{2.8} & \textbf{12.3} & \textbf{73.6} \\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation results on our HybridMatch and HybridLoMatch.  $^{\dagger}$: the model is only trained on 3DMatch. $^{\ddagger}$: the model is trained on our HybridMatch. The best and second-best results are marked in \textbf{bold} and \underline{underlined} for better comparison.}
    \label{tab: DeforMatch_LGR}
\end{table*}

==> tables/DeforMatch_RANSAC.tex <==
\begin{table*}[h]
    \setlength{\tabcolsep}{4.2pt}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|ccccc|ccccc}
        \toprule
        \multirow{4}{*}{\# Samples} & \multicolumn{10}{c|}{HybridMatch} & \multicolumn{10}{c}{HybridLoMatch} \\
        \cmidrule{2-21}
         & \multicolumn{5}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{5}{c|}{\textit{30-50\% non-rigid}} & \multicolumn{5}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{5}{c}{\textit{30-50\% non-rigid}}\\
        \cmidrule{2-21}
        & 5000 & 2500 & 1000 & 500 & 250 & 5000 & 2500 & 1000 & 500 & 250 & 5000 & 2500 & 1000 & 500 & 250 & 5000 & 2500 & 1000 & 500 & 250 \\
        \midrule
        \multicolumn{21}{c}{Feature Matching Recall (\%) $\uparrow$} \\
        \midrule
        PREDATOR & 95.2 & 96.0 & 96.2 & 96.2 & 95.4 & 94.0 & 94.2 & 93.6 & 93.2 & 94.0 & 66.8 & \underline{68.4} & 68.4 & 70.2 & 67.4 & 62.8 & 64.0 & 64.8 & 63.8 & 61.8\\
        CoFiNet & 96.0 & \underline{96.4} & \underline{96.2} & \underline{96.4} & \underline{95.6} & 93.0 & 94.6 & \underline{95.2} & 95.2 & 95.0 & 59.4 & 61.4 & 63.2 & 63.4 & 64.0 & 53.4 & 55.2 & 58.8 & 59.4 & 59.4\\
        GeoTrans & \textbf{99.9} & \textbf{99.8} & \textbf{99.8} & \textbf{99.8} & \textbf{99.8} & \underline{99.4} & \underline{99.4} & \textbf{99.6} & \underline{99.4} & \underline{99.4} & \textbf{93.2} & \textbf{92.8} & \textbf{93.4} & \underline{92.2} & \underline{92.0} & \underline{91.4} & \underline{91.4} & \underline{90.4} & \underline{91.6} & \underline{90.8}\\
        \midrule
        Our \ourmethod{} & \underline{99.8} & \textbf{99.8} & \textbf{99.8} & \textbf{99.8} & \textbf{99.8} & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & \underline{92.8} & \textbf{92.8} & \underline{92.8} & \textbf{92.6} & \textbf{93.0} & \textbf{94.4} & \textbf{94.4} & \textbf{94.8} & \textbf{94.6} & \textbf{94.8}\\
        \midrule
        \multicolumn{21}{c}{Inlier Ratio (\%) $\uparrow$} \\
        \midrule
        PREDATOR & 32.4 & 34.8 & \underline{36.5} & \underline{36.7} & 35.1 & 29.4 & 31.6 & 33.1 & 32.9 & 31.8 & 11.4 & 12.2 & 13.0 & 13.2 & 12.6 & 9.8 & 10.5 & 11.1 & 11.0 & 10.9 \\
        CoFiNet & 23.4 & 26.7 & 31.2 & 32.9 & 34.0 & 21.3 & 24.5 & 28.7 & 30.5 & 31.6 & 7.7 & 8.7 & 10.9 & 11.8 & 12.4 & 7.1 & 7.9 & 9.7 & 10.6 & 11.2 \\
        GeoTrans & \underline{36.5} & \underline{36.5} & 36.4 & \underline{36.7} & \underline{36.4} & \underline{33.6} & \underline{33.6} & \underline{33.7} & \underline{33.6} & \underline{33.6} & \underline{18.2} & \underline{18.3} & \underline{18.3} & \underline{18.3} & \underline{18.4} & \underline{33.6} & \underline{17.3} & \underline{17.4} & \underline{17.3} & \underline{17.2} \\
        \midrule
        Our \ourmethod{} & \textbf{58.6} & \textbf{58.7} & \textbf{58.7} & \textbf{58.8} & \textbf{58.6} & \textbf{54.4} & \textbf{54.4} & \textbf{54.4} & \textbf{54.3} & \textbf{54.3} & \textbf{34.4} & \textbf{34.3} & \textbf{34.3} & \textbf{34.3} & \textbf{34.3} & \textbf{33.8} & \textbf{33.9} & \textbf{33.7} & \textbf{33.7} & \textbf{33.7}  \\
        \midrule
        \multicolumn{21}{c}{Registration Recall (\%) $\uparrow$} \\
        \midrule
        PREDATOR & 65.2 & 73.4 & 79.2 & 80.8 & 80.6 & 57.2 & 69.8 & 74.6 & 75.4 & 71.4 & 19.6 & 26.8 & 33.2 & 32.4 & 30.6& 15.6 & 21.2 & 24.2 & 22.8 & 24.4 \\
        CoFiNet & 79.0 & 80.4 & 82.4 & 80.6 & 79.8 & 75.6 & 78.0 & 77.8 & 77.2 & 72.2 & 27.2 & 27.8 & 29.8 & 27.6 & 27.2 & 21.6 & 24.8 & 25.2 & 25.6 & 24.8 \\
        GeoTrans & \underline{92.8} & \underline{91.4} & \underline{89.0} & \underline{88.6} & \underline{90.0} & \underline{91.0} & \underline{86.8} & \underline{88.6} & \underline{86.8} & \underline{86.4} & \underline{52.6} & \underline{51.4} & \underline{54.4} & \underline{49.2} & \underline{51.8} & \underline{52.4} & \underline{55.2} & \underline{43.8} & \underline{50.0} & \underline{50.8} \\
        \midrule
        Our \ourmethod{} & \textbf{97.4} & \textbf{96.4} & \textbf{97.6} & \textbf{97.2} & \textbf{96.4} & \textbf{96.6} & \textbf{97.4} & \textbf{97.8} & \textbf{95.0} & \textbf{96.0} & \textbf{75.6} & \textbf{73.0} & \textbf{75.2} & \textbf{73.0} & \textbf{70.8} & \textbf{76.2} & \textbf{75.8} & \textbf{75.0} & \textbf{74.2} & \textbf{72.4}  \\
        \bottomrule
    \end{tabular}}
    \caption{Evaluation results on HybridMatch and HybridLoMatch.
    }
    \label{tab: DeforMatch_RANSAC}
\end{table*}

==> tables/ETH.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{9pt}
% \scriptsize
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccc}
        \toprule
        \multicolumn{6}{c}{ETH} \\
        \midrule
        \# Samples & 5000 & 2500 & 1000 & 500 & 250  \\
        \midrule
        PerfectMatch & 81.4 & 73.5 & 59.3 & 46.5 & 35.0 \\
        D3Feat &59.1 & 50.4 & 49.7 & 44.6 & 29.1 \\
        FCGF &42.1 & 36.1 & 29.5 & 26.3 & 18.9 \\
        PREDATOR & 74.7 & 72.9 & 67.7 & 60.3 & 51.7 \\
        CoFiNet & 83.9 & 82.7 & 81.9 & 77.4 & 68.8 \\
        GeoTrans + RANSAC & 80.9 & 76.8 & 73.3 & 72.8 & 70.8 \\
        GeoTrans + LGR  & \multicolumn{2}{c}{\textemdash} & \underline{85.6} & \multicolumn{2}{c}{\textemdash} \\
        \midrule
        Our \ourmethod{} + LGR  & \multicolumn{2}{c}{\textemdash} & \textbf{86.5} & \multicolumn{2}{c}{\textemdash} \\
        \bottomrule
    \end{tabular}}
    \caption{Registration recall comparison on ETH. All models are trained on 3DMatch. %$^{\dagger}$: the model is only trained on the synthetic dataset. $^{\ddagger}$: the model is fine-tuned on 3DMatch. 
    \textemdash: results with different samples are not applicable for LGR since it uses all correspondences.
    % \phil{TODO: Make this table one-column to show only RR and show full results in appendix? Not sure if a careless reviewer will misunderstand when looking at this table}
    }
    \label{tab: ETH}
    % \vspace{-3mm}
\end{table}

==> tables/ablation_DeforMatch_HybridReg.tex <==
\begin{table*}[th]
    \centering
    \setlength{\tabcolsep}{6pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \toprule
         \multirow{4}{*}{Models} & \multicolumn{6}{c|}{HybridMatch} & \multicolumn{6}{c}{HybridLoMatch} \\
         \cmidrule{2-13}
         & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c|}{\textit{30-50\% non-rigid}} & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c}{\textit{30-50\% non-rigid}}\\
         \cmidrule{2-13}
         & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ \\
         \midrule
         (a) Baseline (3D-FRONT) & 2.0 & 8.5 & 52.8 & 2.5 & 12.4 & 44.8 & 4.6 & 16.5 & 18.8 & 4.3 & 19.0 & 14.8 \\
         (b) + Non-rigid Foreground Motion & 1.6 & 7.5 & 90.4 & \underline{2.0} & 9.6 & 86.2 & 3.7 & 14.9 & 54.0 & 4.1 & 16.5 & 48.6 \\
         (c) + Rigid Foreground Motion & \underline{1.4} & \underline{6.0} & \underline{94.0} & \underline{2.0} & \underline{9.4} & \underline{89.2} & \underline{3.5} & \underline{14.1} & \underline{62.8} & \underline{3.3} & \underline{15.4} & \underline{54.2} \\
         (d) + Delete Planes &  \textbf{1.2} &  \textbf{5.4} &  \textbf{97.4} &  \textbf{1.5} &  \textbf{7.1} &  \textbf{96.6} &  \textbf{3.0} &  \textbf{12.2} &  \textbf{75.6} &  \textbf{2.8} &  \textbf{12.3} &  \textbf{73.6} \\
         \midrule
         (e) Baseline (GeoTrans) & \underline{1.4} & \underline{5.6} & 95.6 & \underline{1.6} & 8.1 & 93.6 & \underline{3.3} & \underline{12.3} & 64.2 & \underline{3.2} & 13.7 & 61.0 \\
         (f) w/ Uncertainty Mask + L1 Loss & \underline{1.4} & 5.9 & 94.2 & 1.7 & 8.6 & \underline{95.2} & 3.4 & 13.2 & 66.2 & 3.4 & 15.5 & 61.8 \\
         (g) w/ Uncertainty Mask + NLL Loss & \textbf{1.2} & \textbf{5.4} & \underline{97.2} & \textbf{1.5} & \underline{7.2} & \textbf{96.6} & \textbf{3.0} & \textbf{12.2} & \underline{75.5} & \textbf{2.8} & \underline{12.4} & \underline{73.2} \\
             (h) + Uncertainty-aware Correlation & \textbf{1.2} & \textbf{5.4} & \textbf{97.4} & \textbf{1.5} & \textbf{7.1} & \textbf{96.6} & \textbf{3.0} & \textbf{12.2} & \textbf{75.6} & \textbf{2.8} &  \textbf{12.3} & \textbf{73.6} \\
         \bottomrule
    \end{tabular}}
    \caption{Ablation studies of our proposed \ourdataset{} (top) and \ourmethod{} (bottom).}
    \label{tab: ablation_DeforMatch_HybridReg}
\end{table*}

==> tables/ablation_HybridReg.tex <==
\begin{table*}[th]
    \centering
    % \setlength{\tabcolsep}{2.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \toprule
         \multirow{4}{*}{Methods} & \multicolumn{6}{c|}{DeforMatch} & \multicolumn{6}{c}{DeforLoMatch} \\
         \cmidrule{2-13}
         & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c|}{\textit{30-50\% non-rigid}} & \multicolumn{3}{c|}{\textit{10-30\% non-rigid}} & \multicolumn{3}{c}{\textit{30-50\% non-rigid}}\\
         \cmidrule{2-13}
         & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ & RRE $\downarrow$ & RTE $\downarrow$ & RR $\uparrow$ \\
         \midrule
         (a) Baseline (GeoTrans) & 1.4 & 5.6 & 95.6 & 1.6 & 8.1 & 93.6 & 3.3 & 12.3 & 64.2 & 3.7 & 14.9 & 61.0 \\
         (b) w/ Uncertainty Mask + L1 Loss & 1.4 & 5.9 & 94.2 & 1.7 & 8.6 & 95.2 & 3.4 & 13.2 & 66.2 & 3.5 & 15.1 & 60.5 \\
         (c) w/ Uncertainty Mask + NLL Loss & 1.2 & 5.4 & 97.2 & 1.5 & 7.2 & 96.6 & 3.0 & 12.2 & 75.5 & 2.8 & 13.4 & 73.2 \\
         (d) + Correlation Mask & 1.2 & 5.4 & 97.4 & 1.5 & 7.1 & 96.6 & 3.0 & 12.2 & 75.6 & 2.8 & 13.2 & 73.6 \\
         \bottomrule
    \end{tabular}}
    \caption{Ablation studies of \ourmethod{} on our \ourdataset{}.}
    \label{tab: ablation_HybridReg}
\end{table*}

==> tables/comparison_dataset.tex <==
\begin{table*}[th]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{Datasets} & \multirow{2}{*}{Scene Type} & \multirow{2}{*}{\#Fragments} & \multirow{2}{*}{\#Pairs} & Efficient & Accurate & w/o Human & w/ Rigid & w/ Non-rigid\\
        & & & & Generation & Label & Annotation & Motion & Motion\\
        \midrule 
        3DMatch & real-captured & 3,254 & 20,642 & \XSolidBrush & error-prone & \XSolidBrush & \Checkmark & \XSolidBrush\\
        FlyingShapes & rendering & 21,550 & 107,641 & \Checkmark & accurate & \Checkmark & \Checkmark & \XSolidBrush \\
        PointRegGPT & generative & 320,000 & 160,000 & \XSolidBrush & accurate & \Checkmark & \Checkmark & \XSolidBrush \\
        \midrule 
        Our \ourdataset & rendering & x & x & \Checkmark & accurate & \Checkmark & \Checkmark & \Checkmark \\
        \bottomrule
    \end{tabular}}
    \caption{Comparison among different indoor scene datasets. Existing datasets, \ie, 3DMatch~\cite{zeng20173dmatch}, FlyingShapes~\cite{chen2023sira}, and PointRegGPT~\cite{chen2024pointreggpt} lack diverse deforming foreground motions. Our method can generate large-scale datasets automatically with hybrid motions.}
    \label{tab: comparison_datasets}
\end{table*}
